Neural Lyapunov Model Predictive Control: Learning Safe Global Controllers from Sub-optimal Examples

With a growing interest in data-driven control techniques, Model Predictive Control (MPC) provides an opportunity to exploit the surplus of data reliably, particularly while taking safety and stability into account. In many real-world and industrial applications, it is typical to have an existing control strategy, for instance, execution from a human operator. The objective of this work is to improve upon this unknown, safe but suboptimal policy by learning a new controller that retains safety and stability. Learning how to be safe is achieved directly from data and from a knowledge of the system constraints. The proposed algorithm alternatively learns the terminal cost and updates the MPC parameters according to a stability metric. The terminal cost is constructed as a Lyapunov function neural network with the aim of recovering or extending the stable region of the initial demonstrator using a short prediction horizon. Theorems that characterize the stability and performance of the learned MPC in the bearing of model uncertainties and sub-optimality due to function approximation are presented. The efficacy of the proposed algorithm is demonstrated on non-linear continuous control tasks with soft constraints. The proposed approach can improve upon the initial demonstrator also in practice and achieve better stability than popular reinforcement learning baselines.

==> math_commands.tex <==
% %%%%% NEW MATH DEFINITIONS %%%%%

% \usepackage{amsmath,amsfonts,bm}

% % Mark sections of captions for referring to divisions of figures
% \newcommand{\figleft}{{\em (Left)}}
% \newcommand{\figcenter}{{\em (Center)}}
% \newcommand{\figright}{{\em (Right)}}
% \newcommand{\figtop}{{\em (Top)}}
% \newcommand{\figbottom}{{\em (Bottom)}}
% \newcommand{\captiona}{{\em (a)}}
% \newcommand{\captionb}{{\em (b)}}
% \newcommand{\captionc}{{\em (c)}}
% \newcommand{\captiond}{{\em (d)}}

% % Highlight a newly defined term
% \newcommand{\newterm}[1]{{\bf #1}}


% % Figure reference, lower-case.
% \def\figref#1{Figure~\ref{#1}}
% % Figure reference, capital. For start of sentence
% \def\Figref#1{Figure~\ref{#1}}
% \def\twofigref#1#2{Figures \ref{#1} and \ref{#2}}
% \def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% % Section reference, lower-case.
% \def\secref#1{Section~\ref{#1}}
% % Section reference, capital.
% \def\Secref#1{Section~\ref{#1}}
% % Reference to two sections.
% \def\twosecrefs#1#2{Sections \ref{#1} and \ref{#2}}
% % Reference to three sections.
% \def\secrefs#1#2#3{Sections \ref{#1}, \ref{#2} and \ref{#3}}
% % Reference to an equation, lower-case.
% \def\eqref#1{Equation~\ref{#1}}
% % Reference to an equation, upper case
% \def\Eqref#1{Equation~\ref{#1}}
% % A raw reference to an equation---avoid using if possible
% \def\plaineqref#1{\ref{#1}}
% % Reference to a chapter, lower-case.
% \def\chapref#1{Chapter~\ref{#1}}
% % Reference to an equation, upper case.
% \def\Chapref#1{Chapter~\ref{#1}}
% % Reference to a range of chapters
% \def\rangechapref#1#2{Chapters\ref{#1}--\ref{#2}}
% % Reference to an algorithm, lower-case.
% \def\algref#1{Algorithm~\ref{#1}}
% % Reference to an algorithm, upper case.
% \def\Algref#1{Algorithm~\ref{#1}}
% \def\twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% \def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% % Reference to a part, lower case
% \def\partref#1{Part~\ref{#1}}
% % Reference to a part, upper case
% \def\Partref#1{Part~\ref{#1}}
% \def\twopartref#1#2{Parts \ref{#1} and \ref{#2}}

% \def\ceil#1{\lceil #1 \rceil}
% \def\floor#1{\lfloor #1 \rfloor}
% \def\1{\bm{1}}
% \newcommand{\train}{\mathcal{D}}
% \newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
% \newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

% \def\eps{{\epsilon}}


% % Random variables
% \def\reta{{\textnormal{$\eta$}}}
% \def\ra{{\textnormal{a}}}
% \def\rb{{\textnormal{b}}}
% \def\rc{{\textnormal{c}}}
% \def\rd{{\textnormal{d}}}
% \def\re{{\textnormal{e}}}
% \def\rf{{\textnormal{f}}}
% \def\rg{{\textnormal{g}}}
% \def\rh{{\textnormal{h}}}
% \def\ri{{\textnormal{i}}}
% \def\rj{{\textnormal{j}}}
% \def\rk{{\textnormal{k}}}
% \def\rl{{\textnormal{l}}}
% % rm is already a command, just don't name any random variables m
% \def\rn{{\textnormal{n}}}
% \def\ro{{\textnormal{o}}}
% \def\rp{{\textnormal{p}}}
% \def\rq{{\textnormal{q}}}
% \def\rr{{\textnormal{r}}}
% \def\rs{{\textnormal{s}}}
% \def\rt{{\textnormal{t}}}
% \def\ru{{\textnormal{u}}}
% \def\rv{{\textnormal{v}}}
% \def\rw{{\textnormal{w}}}
% \def\rx{{\textnormal{x}}}
% \def\ry{{\textnormal{y}}}
% \def\rz{{\textnormal{z}}}

% % Random vectors
% \def\rvepsilon{{\mathbf{\epsilon}}}
% \def\rvtheta{{\mathbf{\theta}}}
% \def\rva{{\mathbf{a}}}
% \def\rvb{{\mathbf{b}}}
% \def\rvc{{\mathbf{c}}}
% \def\rvd{{\mathbf{d}}}
% \def\rve{{\mathbf{e}}}
% \def\rvf{{\mathbf{f}}}
% \def\rvg{{\mathbf{g}}}
% \def\rvh{{\mathbf{h}}}
% \def\rvu{{\mathbf{i}}}
% \def\rvj{{\mathbf{j}}}
% \def\rvk{{\mathbf{k}}}
% \def\rvl{{\mathbf{l}}}
% \def\rvm{{\mathbf{m}}}
% \def\rvn{{\mathbf{n}}}
% \def\rvo{{\mathbf{o}}}
% \def\rvp{{\mathbf{p}}}
% \def\rvq{{\mathbf{q}}}
% \def\rvr{{\mathbf{r}}}
% \def\rvs{{\mathbf{s}}}
% \def\rvt{{\mathbf{t}}}
% \def\rvu{{\mathbf{u}}}
% \def\rvv{{\mathbf{v}}}
% \def\rvw{{\mathbf{w}}}
% \def\rvx{{\mathbf{x}}}
% \def\rvy{{\mathbf{y}}}
% \def\rvz{{\mathbf{z}}}

% % Elements of random vectors
% \def\erva{{\textnormal{a}}}
% \def\ervb{{\textnormal{b}}}
% \def\ervc{{\textnormal{c}}}
% \def\ervd{{\textnormal{d}}}
% \def\erve{{\textnormal{e}}}
% \def\ervf{{\textnormal{f}}}
% \def\ervg{{\textnormal{g}}}
% \def\ervh{{\textnormal{h}}}
% \def\ervi{{\textnormal{i}}}
% \def\ervj{{\textnormal{j}}}
% \def\ervk{{\textnormal{k}}}
% \def\ervl{{\textnormal{l}}}
% \def\ervm{{\textnormal{m}}}
% \def\ervn{{\textnormal{n}}}
% \def\ervo{{\textnormal{o}}}
% \def\ervp{{\textnormal{p}}}
% \def\ervq{{\textnormal{q}}}
% \def\ervr{{\textnormal{r}}}
% \def\ervs{{\textnormal{s}}}
% \def\ervt{{\textnormal{t}}}
% \def\ervu{{\textnormal{u}}}
% \def\ervv{{\textnormal{v}}}
% \def\ervw{{\textnormal{w}}}
% \def\ervx{{\textnormal{x}}}
% \def\ervy{{\textnormal{y}}}
% \def\ervz{{\textnormal{z}}}

% % Random matrices
% \def\rmA{{\mathbf{A}}}
% \def\rmB{{\mathbf{B}}}
% \def\rmC{{\mathbf{C}}}
% \def\rmD{{\mathbf{D}}}
% \def\rmE{{\mathbf{E}}}
% \def\rmF{{\mathbf{F}}}
% \def\rmG{{\mathbf{G}}}
% \def\rmH{{\mathbf{H}}}
% \def\rmI{{\mathbf{I}}}
% \def\rmJ{{\mathbf{J}}}
% \def\rmK{{\mathbf{K}}}
% \def\rmL{{\mathbf{L}}}
% \def\rmM{{\mathbf{M}}}
% \def\rmN{{\mathbf{N}}}
% \def\rmO{{\mathbf{O}}}
% \def\rmP{{\mathbf{P}}}
% \def\rmQ{{\mathbf{Q}}}
% \def\rmR{{\mathbf{R}}}
% \def\rmS{{\mathbf{S}}}
% \def\rmT{{\mathbf{T}}}
% \def\rmU{{\mathbf{U}}}
% \def\rmV{{\mathbf{V}}}
% \def\rmW{{\mathbf{W}}}
% \def\rmX{{\mathbf{X}}}
% \def\rmY{{\mathbf{Y}}}
% \def\rmZ{{\mathbf{Z}}}

% % Elements of random matrices
% \def\ermA{{\textnormal{A}}}
% \def\ermB{{\textnormal{B}}}
% \def\ermC{{\textnormal{C}}}
% \def\ermD{{\textnormal{D}}}
% \def\ermE{{\textnormal{E}}}
% \def\ermF{{\textnormal{F}}}
% \def\ermG{{\textnormal{G}}}
% \def\ermH{{\textnormal{H}}}
% \def\ermI{{\textnormal{I}}}
% \def\ermJ{{\textnormal{J}}}
% \def\ermK{{\textnormal{K}}}
% \def\ermL{{\textnormal{L}}}
% \def\ermM{{\textnormal{M}}}
% \def\ermN{{\textnormal{N}}}
% \def\ermO{{\textnormal{O}}}
% \def\ermP{{\textnormal{P}}}
% \def\ermQ{{\textnormal{Q}}}
% \def\ermR{{\textnormal{R}}}
% \def\ermS{{\textnormal{S}}}
% \def\ermT{{\textnormal{T}}}
% \def\ermU{{\textnormal{U}}}
% \def\ermV{{\textnormal{V}}}
% \def\ermW{{\textnormal{W}}}
% \def\ermX{{\textnormal{X}}}
% \def\ermY{{\textnormal{Y}}}
% \def\ermZ{{\textnormal{Z}}}

% % Vectors
% \def\vzero{{\bm{0}}}
% \def\vone{{\bm{1}}}
% \def\vmu{{\bm{\mu}}}
% \def\vtheta{{\bm{\theta}}}
% \def\va{{\bm{a}}}
% \def\vb{{\bm{b}}}
% \def\vc{{\bm{c}}}
% \def\vd{{\bm{d}}}
% \def\ve{{\bm{e}}}
% \def\vf{{\bm{f}}}
% \def\vg{{\bm{g}}}
% \def\vh{{\bm{h}}}
% \def\vi{{\bm{i}}}
% \def\vj{{\bm{j}}}
% \def\vk{{\bm{k}}}
% \def\vl{{\bm{l}}}
% \def\vm{{\bm{m}}}
% \def\vn{{\bm{n}}}
% \def\vo{{\bm{o}}}
% \def\vp{{\bm{p}}}
% \def\vq{{\bm{q}}}
% \def\vr{{\bm{r}}}
% \def\vs{{\bm{s}}}
% \def\vt{{\bm{t}}}
% \def\vu{{\bm{u}}}
% \def\vv{{\bm{v}}}
% \def\vw{{\bm{w}}}
% \def\vx{{\bm{x}}}
% \def\vy{{\bm{y}}}
% \def\vz{{\bm{z}}}

% % Elements of vectors
% \def\evalpha{{\alpha}}
% \def\evbeta{{\beta}}
% \def\evepsilon{{\epsilon}}
% \def\evlambda{{\lambda}}
% \def\evomega{{\omega}}
% \def\evmu{{\mu}}
% \def\evpsi{{\psi}}
% \def\evsigma{{\sigma}}
% \def\evtheta{{\theta}}
% \def\eva{{a}}
% \def\evb{{b}}
% \def\evc{{c}}
% \def\evd{{d}}
% \def\eve{{e}}
% \def\evf{{f}}
% \def\evg{{g}}
% \def\evh{{h}}
% \def\evi{{i}}
% \def\evj{{j}}
% \def\evk{{k}}
% \def\evl{{l}}
% \def\evm{{m}}
% \def\evn{{n}}
% \def\evo{{o}}
% \def\evp{{p}}
% \def\evq{{q}}
% \def\evr{{r}}
% \def\evs{{s}}
% \def\evt{{t}}
% \def\evu{{u}}
% \def\evv{{v}}
% \def\evw{{w}}
% \def\evx{{x}}
% \def\evy{{y}}
% \def\evz{{z}}

% % Matrix
% \def\mA{{\bm{A}}}
% \def\mB{{\bm{B}}}
% \def\mC{{\bm{C}}}
% \def\mD{{\bm{D}}}
% \def\mE{{\bm{E}}}
% \def\mF{{\bm{F}}}
% \def\mG{{\bm{G}}}
% \def\mH{{\bm{H}}}
% \def\mI{{\bm{I}}}
% \def\mJ{{\bm{J}}}
% \def\mK{{\bm{K}}}
% \def\mL{{\bm{L}}}
% \def\mM{{\bm{M}}}
% \def\mN{{\bm{N}}}
% \def\mO{{\bm{O}}}
% \def\mP{{\bm{P}}}
% \def\mQ{{\bm{Q}}}
% \def\mR{{\bm{R}}}
% \def\mS{{\bm{S}}}
% \def\mT{{\bm{T}}}
% \def\mU{{\bm{U}}}
% \def\mV{{\bm{V}}}
% \def\mW{{\bm{W}}}
% \def\mX{{\bm{X}}}
% \def\mY{{\bm{Y}}}
% \def\mZ{{\bm{Z}}}
% \def\mBeta{{\bm{\beta}}}
% \def\mPhi{{\bm{\Phi}}}
% \def\mLambda{{\bm{\Lambda}}}
% \def\mSigma{{\bm{\Sigma}}}

% % Tensor
% \DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
% \SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
% \newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
% \def\tA{{\tens{A}}}
% \def\tB{{\tens{B}}}
% \def\tC{{\tens{C}}}
% \def\tD{{\tens{D}}}
% \def\tE{{\tens{E}}}
% \def\tF{{\tens{F}}}
% \def\tG{{\tens{G}}}
% \def\tH{{\tens{H}}}
% \def\tI{{\tens{I}}}
% \def\tJ{{\tens{J}}}
% \def\tK{{\tens{K}}}
% \def\tL{{\tens{L}}}
% \def\tM{{\tens{M}}}
% \def\tN{{\tens{N}}}
% \def\tO{{\tens{O}}}
% \def\tP{{\tens{P}}}
% \def\tQ{{\tens{Q}}}
% \def\tR{{\tens{R}}}
% \def\tS{{\tens{S}}}
% \def\tT{{\tens{T}}}
% \def\tU{{\tens{U}}}
% \def\tV{{\tens{V}}}
% \def\tW{{\tens{W}}}
% \def\tX{{\tens{X}}}
% \def\tY{{\tens{Y}}}
% \def\tZ{{\tens{Z}}}


% % Graph
% \def\gA{{\mathcal{A}}}
% \def\gB{{\mathcal{B}}}
% \def\gC{{\mathcal{C}}}
% \def\gD{{\mathcal{D}}}
% \def\gE{{\mathcal{E}}}
% \def\gF{{\mathcal{F}}}
% \def\gG{{\mathcal{G}}}
% \def\gH{{\mathcal{H}}}
% \def\gI{{\mathcal{I}}}
% \def\gJ{{\mathcal{J}}}
% \def\gK{{\mathcal{K}}}
% \def\gL{{\mathcal{L}}}
% \def\gM{{\mathcal{M}}}
% \def\gN{{\mathcal{N}}}
% \def\gO{{\mathcal{O}}}
% \def\gP{{\mathcal{P}}}
% \def\gQ{{\mathcal{Q}}}
% \def\gR{{\mathcal{R}}}
% \def\gS{{\mathcal{S}}}
% \def\gT{{\mathcal{T}}}
% \def\gU{{\mathcal{U}}}
% \def\gV{{\mathcal{V}}}
% \def\gW{{\mathcal{W}}}
% \def\gX{{\mathcal{X}}}
% \def\gY{{\mathcal{Y}}}
% \def\gZ{{\mathcal{Z}}}

% % Sets
% \def\sA{{\mathbb{A}}}
% \def\sB{{\mathbb{B}}}
% \def\sC{{\mathbb{C}}}
% \def\sD{{\mathbb{D}}}
% % Don't use a set called E, because this would be the same as our symbol
% % for expectation.
% \def\sF{{\mathbb{F}}}
% \def\sG{{\mathbb{G}}}
% \def\sH{{\mathbb{H}}}
% \def\sI{{\mathbb{I}}}
% \def\sJ{{\mathbb{J}}}
% \def\sK{{\mathbb{K}}}
% \def\sL{{\mathbb{L}}}
% \def\sM{{\mathbb{M}}}
% \def\sN{{\mathbb{N}}}
% \def\sO{{\mathbb{O}}}
% \def\sP{{\mathbb{P}}}
% \def\sQ{{\mathbb{Q}}}
% \def\sR{{\mathbb{R}}}
% \def\sS{{\mathbb{S}}}
% \def\sT{{\mathbb{T}}}
% \def\sU{{\mathbb{U}}}
% \def\sV{{\mathbb{V}}}
% \def\sW{{\mathbb{W}}}
% \def\sX{{\mathbb{X}}}
% \def\sY{{\mathbb{Y}}}
% \def\sZ{{\mathbb{Z}}}

% % Entries of a matrix
% \def\emLambda{{\Lambda}}
% \def\emA{{A}}
% \def\emB{{B}}
% \def\emC{{C}}
% \def\emD{{D}}
% \def\emE{{E}}
% \def\emF{{F}}
% \def\emG{{G}}
% \def\emH{{H}}
% \def\emI{{I}}
% \def\emJ{{J}}
% \def\emK{{K}}
% \def\emL{{L}}
% \def\emM{{M}}
% \def\emN{{N}}
% \def\emO{{O}}
% \def\emP{{P}}
% \def\emQ{{Q}}
% \def\emR{{R}}
% \def\emS{{S}}
% \def\emT{{T}}
% \def\emU{{U}}
% \def\emV{{V}}
% \def\emW{{W}}
% \def\emX{{X}}
% \def\emY{{Y}}
% \def\emZ{{Z}}
% \def\emSigma{{\Sigma}}

% % entries of a tensor
% % Same font as tensor, without \bm wrapper
% \newcommand{\etens}[1]{\mathsfit{#1}}
% \def\etLambda{{\etens{\Lambda}}}
% \def\etA{{\etens{A}}}
% \def\etB{{\etens{B}}}
% \def\etC{{\etens{C}}}
% \def\etD{{\etens{D}}}
% \def\etE{{\etens{E}}}
% \def\etF{{\etens{F}}}
% \def\etG{{\etens{G}}}
% \def\etH{{\etens{H}}}
% \def\etI{{\etens{I}}}
% \def\etJ{{\etens{J}}}
% \def\etK{{\etens{K}}}
% \def\etL{{\etens{L}}}
% \def\etM{{\etens{M}}}
% \def\etN{{\etens{N}}}
% \def\etO{{\etens{O}}}
% \def\etP{{\etens{P}}}
% \def\etQ{{\etens{Q}}}
% \def\etR{{\etens{R}}}
% \def\etS{{\etens{S}}}
% \def\etT{{\etens{T}}}
% \def\etU{{\etens{U}}}
% \def\etV{{\etens{V}}}
% \def\etW{{\etens{W}}}
% \def\etX{{\etens{X}}}
% \def\etY{{\etens{Y}}}
% \def\etZ{{\etens{Z}}}

% % The true underlying data generating distribution
% \newcommand{\pdata}{p_{\rm{data}}}
% % The empirical distribution defined by the training set
% \newcommand{\ptrain}{\hat{p}_{\rm{data}}}
% \newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% % The model distribution
% \newcommand{\pmodel}{p_{\rm{model}}}
% \newcommand{\Pmodel}{P_{\rm{model}}}
% \newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% % Stochastic autoencoder distributions
% \newcommand{\pencode}{p_{\rm{encoder}}}
% \newcommand{\pdecode}{p_{\rm{decoder}}}
% \newcommand{\precons}{p_{\rm{reconstruct}}}

% \newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

% \newcommand{\E}{\mathbb{E}}
% \newcommand{\Ls}{\mathcal{L}}
% \newcommand{\R}{\mathbb{R}}
% \newcommand{\emp}{\tilde{p}}
% \newcommand{\lr}{\alpha}
% \newcommand{\reg}{\lambda}
% \newcommand{\rect}{\mathrm{rectifier}}
% \newcommand{\softmax}{\mathrm{softmax}}
% \newcommand{\sigmoid}{\sigma}
% \newcommand{\softplus}{\zeta}
% \newcommand{\KL}{D_{\mathrm{KL}}}
% \newcommand{\Var}{\mathrm{Var}}
% \newcommand{\standarderror}{\mathrm{SE}}
% \newcommand{\Cov}{\mathrm{Cov}}
% % Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% % But then they seem to use $L^2$ for vectors throughout the site, and so does
% % wikipedia.
% \newcommand{\normlzero}{L^0}
% \newcommand{\normlone}{L^1}
% \newcommand{\normltwo}{L^2}
% \newcommand{\normlp}{L^p}
% \newcommand{\normmax}{L^\infty}

% \newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}

% \DeclareMathOperator{\sign}{sign}
% \DeclareMathOperator{\Tr}{Tr}
% \let\ab\allowbreak

